WhiteLie: A Robust System for Spoofing User Data in Android Platforms

Android employs a permission framework that empowers users to either accept or deny sharing their private data (for example, location) with an app. However, many apps tend to crash when they are denied permission, leaving users no choice but to allow access to their data in order to use the app. In this paper, we introduce a comprehensive and robust user data spoofing system, WhiteLie, that can spoof a variety of user data and feed it to target apps. Additionally, it detects privacy-violating behaviours, automatically responding by supplying spoofed data instead of the user's real data, without crashing or disrupting the apps. Unlike prior approaches, WhiteLie requires neither device rooting nor altering the app's binary, making it deployable on stock Android devices. Through experiments on more than 70 popular Android apps, we demonstrate that WhiteLie is able to deceive apps into accepting spoofed data without getting detected. Our evaluation further demonstrates that WhiteLie introduces negligible overhead in terms of battery usage, CPU consumption, and app execution latency. Our findings underscore the feasibility of implementing user-centric privacy-enhancing mechanisms within the existing Android ecosystem.

==> listings/battery_saver.tex <==
\begin{lstlisting}[caption={Kotlin code to save battery by returning \texttt{null} based on \texttt{batterySaver} policy defined by user},label={lst:btrySvr},language=Kotlin]
override fun beforeHookedMethod(_:MethodHookParam){
    val cursor = getDeceitSettings() 
    val bs = getString(cursor, "batterySaver")
    if(bs == "true") return null
    cursor.close()
}
\end{lstlisting}

==> listings/hooking_mechanism.tex <==
\begin{lstlisting}[caption={Kotlin code to hook target method ``\textit{methodName}" of class ``\textit{ClassName}" using Xposed Framework},label={lst:hooking},language=Kotlin]
XposedHelpers.findAndHookMethod(
  "ClassName", 
  lpparam.classLoader, 
  "methodName", 
  XC_MethodHook() {
    @Throws(Throwable::class)
    override protected void beforeHookedMethod(
      MethodHookParam param) {
        super.beforeHookedMethod(param)
    }

    @Throws(Throwable::class)
    override protected void afterHookedMethod(
      MethodHookParam param) {
        super.afterHookedMethod(param)
    }
  }
)
\end{lstlisting}

==> tables/experiments_strategy.tex <==
\begin{table}[htbp]
    \caption{Benchmarking and Deceiving Strategy used for each permission while evaluating performance overhead }
    {\tiny
    \begin{center}
        % \begin{threeparttable}
            \begin{tabular}{|>{\centering}m{0.15\linewidth}|m{0.4\linewidth}|m{0.26\linewidth}|}
                \hline
                \textbf{Permission} & \textbf{\textit{Bench-marking Strategy}} & \textbf{\textit{Deceived by}} \\
                \hline
                Calendar & Calls \texttt{ContentProvider. query()} for calendar events and traverse. & a database cursor with 30 fake calendar events rows.\\
                \hline
                Call Log & Calls \texttt{ContentProvider. query()} API for call logs and traverse. & a cursor to the database with 30 fake call logs. \\
                \hline
                Camera & Display the camera stream preview frame using \texttt{camera2} API. & the preview frame with a black image of same resolution. \\
                \hline
                Clipboard & Sets text of a \texttt{textView} with \texttt{ClipboardManager.prim- aryClip} text & a random string generated of arbitrary size.  \\
                \hline
                Contacts & Calls \texttt{ContentProvider. query()} API for contacts and traverse. & a cursor to the database with 30 fake contacts. \\
                \hline
                Location & Calls \texttt{LocationManager. getLastKnownLocation()} and logs the lats and longs & randomly generated float values  for lats and longs\\
                \hline
                Messages & Calls \texttt{ContentProvider. query()} API for messages and traverse. & a cursor to the database with 30 fake messages. \\
                \hline
                Network & \texttt{WifiManager.getConnec- tionInfo()} is called to log information like SSID. & randomly generated strings of arbitrary size. \\
                \hline
                Packages &  Calls \texttt{PackageManager. getInstalledPackages()} API and traverses over the list. & a list of 25 deceived packages \texttt{PackageInfo}. \\
                \hline
                Tracking & Logs various information fetched using \texttt{Telephony- Manager.getString()}. & randomly generated strings satisfying the patterns.  \\
                \hline
            \end{tabular}
            % \begin{tablenotes}
            %     \item[1] To maintain the consistency before and after deceiving the permission, the number of rows in the cursor returned by the \texttt{query()} method was maintained to be 30.
            %     \item[2] To maintain the consistency before and after deceiving the permission, after deceiving the permission, \framework{} was modified to return the first 25 packages as deceived and the rest as returned by the non-hooked method call.
            % \end{tablenotes}
        %  \end{threeparttable}
    \end{center}
    }
    \label{tab:benchmarking_strategy}
\end{table}
